jina-embeddings-v3: Multilingual Embeddings With Task LoRA

We introduce jina-embeddings-v3, a novel text embedding model with 570 million parameters, achieves state-of-the-art performance on multilingual data and long-context retrieval tasks, supporting context lengths of up to 8192 tokens. The model includes a set of task-specific Low-Rank Adaptation (LoRA) adapters to generate high-quality embeddings for query-document retrieval, clustering, classification, and text matching. Evaluation on the MTEB benchmark shows that jina-embeddings-v3 outperforms the latest proprietary embeddings from OpenAI and Cohere on English tasks, while achieving superior performance compared to multilingual-e5-large-instruct across all multilingual tasks. With a default output dimension of 1024, users can flexibly reduce the embedding dimensions to as low as 32 without compromising performance, enabled by Matryoshka Representation Learning.

==> tables/ablation_study_sts.tex <==
\begin{tabular}{llcccccccccc}
     \toprule
     Lang. & Variant & BIOSSES & SICK-R* & STS12* & STS13 & STS14 & STS15 & STS16 & STS17 & STS22  \\
     \midrule
     \multirow{3}{*}{de} 
      & Pearson  & 0.780 &  \bfseries 0.811 & \bfseries 0.801 & \bfseries 0.851 & 0.811 & \bfseries 0.878 & 0.836 & \bfseries 0.893 & \bfseries 0.682 \\
      & MSE & 0.784 & 0.793 & 0.797 & 0.849 & \bfseries 0.812 & 0.874 & \bfseries 0.842 & 0.892 & 0.677 \\
      & No STS data & \bfseries 0.797 & 0.791 & 0.792 & 0.847 & 0.810 & 0.876 & 0.839  & 0.890 & 0.676 \\
     \midrule
     \multirow{ 3}{*}{es} 
     & Pearson & \bfseries 0.830 & \bfseries 0.830 & \bfseries 0.816 & \bfseries 0.868 & \bfseries 0.836 & \bfseries 0.887 & \bfseries 0.860 & \bfseries 0.886 & 0.656 \\
     & MSE & 0.825 & 0.801 & 0.810 & 0.867 & 0.834 & \bfseries 0.887 & \bfseries 0.860 & 0.884 &     0.657 \\
     & No STS data & 0.825 &  0.792 & 0.801 & 0.866 & 0.831 & 0.882 & 0.855 & 0.882 & \bfseries 0.662 \\ 
     \bottomrule
\end{tabular}

==> tables/english/average_per_task.tex <==
\begin{tabular}{lcccccccc}
 \toprule
 Model & Average & CF & CL & PC & RR & RT & STS & SM \\
 \midrule
    jina-embeddings-v3 & 65.60 & \textbf{82.57} & 45.37 & 84.00 & 57.94 & 53.87 & \textbf{86.14} & 30.98 \\
    text-embedding-3-large & 62.03 & 75.45 & 49.01 & 84.22 & 59.16 & 55.44 & 81.04 & 29.92 \\
    multilingual-e5-large-instruct & 64.41 & 77.56 & 47.1 & 86.19 & 58.58 & 52.47 & 48.78 & 30.39 \\
    Cohere-embed-multilingual-v3.0 & 60.08 & 64.01 & 46.60 & 86.15 & 57.86 & 53.84 & 83.15 & 30.99 \\
    % English-only models
    % gte-large-en & 65.39 & 77.75 & \textbf{47.96} & 84.53 & 58.5 & \textbf{57.91} & 81.43 & 30.91 \\
    % cohere-embed-english & 64.47 & 76.49 & 47.43 & 85.84 & 58.01 & 55.00 & 82.62 & 30.18 \\
    % gecko-text-embedding & \textbf{66.31} & 81.17 & 47.48 & \textbf{87.61} & \textbf{58.90} & 55.70 & 85.07 & \textbf{32.63} \\
 \bottomrule
\end{tabular}

==> tables/english/classification.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & Cohere-embed-multilingual-v3 \\
\midrule
mean & 82.58 & 75.45 & 77.56 & 76.01 \\
AmazonCounterfactualClassification & 89.49 & 78.83 & 76.24 & 77.85 \\
AmazonPolarityClassification & 95.38 & 92.85 & 96.29 & 95.60 \\
AmazonReviewsClassification & 49.74 & 48.7 & 56.72 & 49.79 \\
Banking77Classification (en) & 84.08 & 85.69 & 85.73 & 86.09 \\
EmotionClassification (en) & 73.33 & 51.58 & 51.51 &  48.15\\
ImdbClassification (en) & 91.90 & 87.67 & 94.60 & 93.97 \\
MTOPDomainClassification (en) & 97.49 & 95.36 & 93.93 & 94.92 \\
MTOPIntentClassification (en) & 84.55 & 75.05 & 82.46 & 78.89 \\
MassiveIntentClassification (en) & 77.6 & 74.64 & 77.06 & 74.51 \\
MassiveScenarioClassification (en) & 84.71 & 79.79 & 80.47 & 79.00 \\
ToxicConversationsClassification (en) & 91.28 & 72.92 & 71.06 & 71.20 \\
TweetSentimentExtractionClassification (en) & 71.39 & 62.22 & 64.62 & 62.18 \\
\bottomrule
\end{tabular}

==> tables/english/clustering.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean & 45.21 & 49.00 & 47.10 & 46.60 \\
ArxivClusteringP2P (en) & 46.66 & 49.01 & 46.40 & 48.16 \\
ArxivClusteringS2S (en) & 38.19 & 44.45 & 40.49 & 40.79 \\
BiorxivClusteringP2P (en) & 34.42 & 38.03 & 40.94 & 40.50 \\
BiorxivClusteringS2S (en) & 32.42 & 36.53 & 36.28 & 36.91 \\
MedrxivClusteringP2P (en) & 34.71 & 32.70 & 36.93 & 36.18 \\
MedrxivClusteringS2S (en) & 32.48 & 31.27 & 35.54 & 33.44 \\
RedditClustering (en) & 55.64 & 67.84 & 56.60 & 58.11 \\
RedditClusteringP2P (en) & 63.31 & 67.96 & 64.27 & 65.02 \\
StackExchangeClustering (en) & 66.15 & 76.26 & 66.85 & 68.12 \\
StackExchangeClusteringP2P (en) & 35.40 & 36.88 & 42.46 & 35.22 \\
TwentyNewsgroupsClustering (en) & 52.42 & 58.14 & 51.33 & 50.14 \\
\bottomrule
\end{tabular}


==> tables/english/pair-classification.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean & 84.01 & 84.22 & 86.19 & 	86.15 \\
SprintDuplicateQuestions (en) & 96.98 & 89.02 & 91.18 & 96.79 \\
TwitterSemEval2015 (en) & 70.91 & 76.56 & 80.27 & 75.16 \\
TwitterURLCorpus (en) & 84.13 & 87.09 & 87.12 & 86.49 \\
\bottomrule
\end{tabular}


==> tables/english/reranking.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean &  &  &  &  \\
AskUbuntuDupQuestions (en) &  &  &  &  \\
MindSmallReranking (en) &  &  &  &  \\
SciDocsRR (en) &  &  &  &  \\
StackOverflowDupQuestions (en) &  &  &  &  \\
\bottomrule
\end{tabular}


==> tables/english/retrieval.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean & 53.96 & 55.44 & 52.47 & 53.84 \\
ArguAna (en) & 57.69 & 58.05 & 58.38 & 55.11 \\
CQADupstackRetrieval (en) & 40.03 & 47.54 & 42.71 & 40.64 \\
ClimateFEVER (en) & 42.38 & 30.27 & 29.86 & 29.96 \\
DBPedia (en) & 41.08 & 44.76 & 38.36 & 41.00 \\
FEVER (en) & 89.04 & 87.94 & 77.99 & 88.53 \\
FiQA2018 (en) & 47.33 & 55.00 & 47.71 & 44.10 \\
HotpotQA (en) & 64.64 & 71.58 & 69.32 & 70.61 \\
MSMARCO (en) & 40.81 & 40.24 & 40.43 & 43.45 \\
NFCorpus (en) & 36.59 & 42.07 & 35.53 & 36.42 \\
NQ (en) & 64.31 & 61.27 & 57.75 & 63.41 \\
QuoraRetrieval (en) & 88.90 & 89.05 & 89.15 & 88.92 \\
SCIDOCS (en) & 19.84 & 23.11 & 18.72 & 19.34 \\
SciFact (en) & 72.72 & 77.77 & 71.85 & 70.05 \\
TRECCOVID (en) & 77.67 & 79.56 & 82.00 & 83.37 \\
Touche2020 (en) & 26.30 & 23.35 & 27.25 & 32.70 \\
\bottomrule
\end{tabular}


==> tables/english/sts.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean & 86.14 & 81.04 & 84.78 & 83.15 \\
BIOSSES & 86.98 & 84.87 & 86.96 & 85.01 \\
SICK-R & 89.04 & 79.18 & 81.73 & 82.18 \\
STS12 & 82.46 & 71.98 & 82.57 & 77.62 \\
STS13 & 89.97 & 85.52 & 87.15 & 85.16 \\
STS14 & 86.82 & 80.50 & 84.97 & 80.02 \\
STS15 & 90.74 & 87.51 & 91.05 & 88.92 \\
STS16 & 86.91 & 84.48 & 87.31 & 86.92 \\
STS17 (en-en) & 90.76 & 88.11 & 90.03 & 90.09 \\
STS22 (en) & 67.95 & 65.92 & 67.63 & 66.81 \\
STSBenchmark & 89.77 & 82.34 & 88.38 & 88.79 \\
\bottomrule
\end{tabular}

==> tables/english/summarization.tex <==
\begin{tabular}{lcccc}
\toprule
 & jina-embeddings-v3 & text-embedding-3-large & multilingual-e5-large-instruct & cohere-embed-multilingual-v3 \\
\midrule
mean & 30.89 & 29.92 & 30.39 & 30.99 \\
SummEval  & 30.89 & 29.92 & 30.39 & 30.99 \\
\bottomrule
\end{tabular}


==> tables/multilingual/average.tex <==
\begin{tabular}{lcccccccc}
 \toprule
 Model & Average & CF & CL & PC & RR & RT & STS & SM \\
 \midrule
    jina-embeddings-v2 &  & 65.90 & 40.14 & 82.95 & 66.57 & 53.42 &  &  \\
    jina-embeddings-v3 &  & 72.11 & 47.52 & 72.95 & 65.36 & 57.58 &  &  \\
    multilingual-e5-large &  & 65.26 & 43.11 & 72.49 & 67.91 &  & 70.27 &  \\
 \bottomrule
\end{tabular}

==> tables/multilingual/summarization.tex <==
\begin{tabular}{lcccccc}
\toprule
 & je-v2 & je-v3 & m-e5-large & te-3-large & cohere-text & m-e5-instr \\
 \midrule
Summarization Average [Spearman] &  &  \\
SummEval &  &  \\
\bottomrule
\end{tabular}
